Dark Energy Survey Year 3 Results: Weak Lensing Shape Catalogue

We present and characterise the galaxy shape catalogue from the first 3 years of Dark Energy Survey (DES) observations, over an effective area of ~4143 deg$^2$ of the southern sky. We describe our data analysis process and our self-calibrating shear measurement pipeline METACALIBRATION, which builds and improves upon the pipeline used in the DES Year 1 analysis in several aspects. The DES Year 3 weak-lensing shape catalogue consists of 100,204,026 galaxies, measured in the $riz$ bands, resulting in a weighted source number density of $n_{\rm eff} = 5.59$ gal/arcmin$ ^{2}$ and corresponding shape noise $\sigma_e = 0.261$. We perform a battery of internal null tests on the catalogue, including tests on systematics related to the point-spread function (PSF) modelling, spurious catalogue B-mode signals, catalogue contamination, and galaxy properties.

==> Makefile <==

texfile := main
default: pdf

# just run it
bib: 
	bibtex ${texfile}

pdf:
	pdflatex ${texfile}

clean:
	rm -f \
	${texfile}.dvi \
	${texfile}.out \
	${texfile}.ps \
	${texfile}.pdf \
	${texfile}.aux \
	${texfile}.bbl \
	${texfile}.blg \
	${texfile}.toc \
	${texfile}.log

